LLM-AutoDiff: Auto-Differentiate Any LLM Workflow

Large Language Models (LLMs) have reshaped natural language processing, powering applications from multi-hop retrieval and question answering to autonomous agent workflows. Yet, prompt engineering -- the task of crafting textual inputs to effectively direct LLMs -- remains difficult and labor-intensive, particularly for complex pipelines that combine multiple LLM calls with functional operations like retrieval and data formatting. We introduce LLM-AutoDiff: a novel framework for Automatic Prompt Engineering (APE) that extends textual gradient-based methods (such as Text-Grad) to multi-component, potentially cyclic LLM architectures. Implemented within the AdalFlow library, LLM-AutoDiff treats each textual input as a trainable parameter and uses a frozen backward engine LLM to generate feedback-akin to textual gradients -- that guide iterative prompt updates. Unlike prior single-node approaches, LLM-AutoDiff inherently accommodates functional nodes, preserves time-sequential behavior in repeated calls (e.g., multi-hop loops), and combats the "lost-in-the-middle" problem by isolating distinct sub-prompts (instructions, formats, or few-shot examples). It further boosts training efficiency by focusing on error-prone samples through selective gradient computation. Across diverse tasks, including single-step classification, multi-hop retrieval-based QA, and agent-driven pipelines, LLM-AutoDiff consistently outperforms existing textual gradient baselines in both accuracy and training cost. By unifying prompt optimization through a graph-centric lens, LLM-AutoDiff offers a powerful new paradigm for scaling and automating LLM workflows - mirroring the transformative role that automatic differentiation libraries have long played in neural network research.

==> tex/abstract.tex <==
\begin{abstract}

    % Prompt optimization is a discret optimization problem, yet similar to the continous optimization, the search space is vast and the optimization is np hard. 
    % In some way, few-shot learning where the we select a few examples as a few-shot demonstration in the context is a subset of the prompt optimization, where the search space is vastly reduced.
    % The current leading auto-prompt optimization in APE with the most prompising benchmarks is Text Grad, which is a analog to the gradient descent in the continous optimization where the weights are prompts, the numerical gradients are becoming textual feedback given by an LLM called "backward engine", and the optimizer is another LLM taking the feedback, current values, and optionally all past iterations to propose a new prompt, all based on a textual loss function with an evaluation function.
    % As LLM applications such as chatbots, RAGs, and agent are a compound system which can be represented as a graph, the future of the prompt optimization largely lies in this direction. 
    % We have three main contributions in this paper where for the first time, we have a systemtic structure in `AdalFlow' library similar to how `PyTorch' and `PyTorch' can almost automatically any combination of basic neural networks, either rnns, cnns, transformers, it can all be auto-differentiated.

    % (1) Similar to the auto-differentiation, the loss is only accumulated from training samples that has error, while in most cases, the manual prompt we start with can give us an accuracy, e.g. 70\% accuracy, so we propose to only use the backward engine to give to the samples that has errors.
    % We found it not only speed up the training, lower the token cost, but also improve the accuracy.
    % (2) Similra to RNN where there are cycles, for agents or multi-hop RAG where there are also cycles, we propose similar approaches to handle this: (a) we can expand the cycle into multiple nodes which are multiple copies. but this method cant be applied in cycles where the number of nodes are not fixed, e.g. a cycle with a variable number of nodes, so we propose (b) use the same prompt, and as it cycles, we accumlate the feedbacks and update the prompt as if it has $n$ sets of input-output pairs, where $n$ is the number of cycles. 
    % (3) Previous research did both random minimum batch and beam search where it generates multiple proposals of prompts and use complicated heuristic search, we propos "moving minimum batch" where we create a minmum set of more balanced correct and error samples, and we loop $k$ times to create $k$ variants of proposals and pass a three stage of validations.
    % (a) the first is the minimum set, if the proposed prompt can not even "decrease the training loss", it is rejected. (b) the second is the whole moving minimum batch, where other samples besides of the selected minimum set has not contributed to the training, this is a minimum random samling of the whole validation set, if the proposed prompt will be rejected if the accuracy is not improved. (c) the third is the whole validation set, where the proposed prompt will be rejected if the accuracy is not improved.
    % (4) Last, we combine with Few-shot learning to train in the same LLM prompt. We also found that a prompt consides of multiple types of subprompts, such as the task instruction, output format, the few-shot, the tool use, the context from retrieval, it becomes too complicated for "backward engine" and the "LLM optimizer" to handle all at once, and we proposed to separate them into different Parameters and to avoid "cross-contamination" between them, we propose "peer nodes" in the dynamic computetion of text grad.
    % We introduce automatic differentiation for multi-node systems within the AdalFlow library, extending textual gradient-based methods (e.g., Text-Grad) to more complex, multi-component LLM systems. 
    We introduce \textbf{LLM-Diff}, a novel framework for \textit{Automatic Prompt Engineering (APE)} implemented in AdalFlow~\footnote{\url{https://github.com/SylphAI-Inc/AdalFlow}
        is a powerful and easy to use LLM library with many basic building blocks for developers and researchers to buld and auto-optimize LLM applications such as chatbots, RAGs, and agents.
    } that extends textual gradient-based methods (e.g., Text-Grad) to more complex, multi-component LLM systems.
    % We introduce automatic differentiation for multi-node LLM systems within the AdalFlow library. 
    LLM-Diff models an LLM application as a directed (potentially cyclic) graph of components—LLMs, retrievers, and other functional components—then builds a corresponding runtime computation(“parameter") graph to propagate textual gradients.
    By employing a frozen “backward engine” LLM for gradient generation and a separate “optimizer” LLM for prompt updates,
    LLM-Diff automates prompt tuning in a flexible, modular way.
    Our contributions are two folds. 1. A comphrensive approach on auto-differentiate any compound LLM system by introducing \textbf{Pass-Through Gradients} to
    handle functional but non-trainable intermediate components, \textbf{Time-Sequential Gradients} to handle cycles in the graph.
    2. Efficient training methods including (1) computing gradients for all peers in a single backward pass, (2) only on training samples with ``errors'', (3) and validate multiple proposals for each backward pass first on the mini-batch, and only on the whole validation set if the accuracy is improved.
    
    Empirical results on one-node, multi-node, cyclic, and agentic applications demonstrate that LLM-Diff achieves faster convergence, higher accuracy, and reduced token consumption compared to baseline prompt-engineering approaches, offering a scalable solution for complex LLM-based systems.
\end{abstract}

% Our main contributions are: (1) \textbf{Gradient Pass-Through.} We introduce a mechanism for passing gradients through purely functional intermediate nodes,
    % enabling end-to-end optimization across multi-node systems.
    % (2) \textbf{Cyclic Structure Handling.} We handle cyclical graphs (e.g., multi-hop RAG or iterative agents) by tracking and ordering gradients over repeated node calls, preserving their runtime sequence.
    % (3) \textbf{Peer Nodes.} We propose “peer nodes” to optimize multiple subprompts (e.g., task instructions, few-shot examples, output format) within the same LLM call, preventing cross-contamination among subprompts and improve optimization effectiveness.
    % (4) \textbf{Selective Gradient Computation.} We compute gradients only for samples with errors, reducing token usage while emphasizing the most informative training signals.





==> tex/introduction_new.tex <==
% \section{Introduction}

% \textbf{LLM apps with chatbots, rags, and agents}
% Large Langage models(LLMs)'s emerging in-context learning capabilities~\cite{brown2020language} has taken the whole world by storm, 
% nearly all product teams and academic institutions are researching and building LLM apps.
% We see these LLM applications such as Chatbots~\cite{}, RAGs~\cite{khattab2022demonstrate}, and agents~\cite{yao2022react} to replace the traditionally rule-based software system, changing both the front-end and back-end of the software system.
% There are emerging prompt engineering methods~\cite{wei2022chain,shinn2024reflexion } for developers and researchers to optimize the applications.
% Prompting is much needed and highly effective at adapting any LLM model to the downstream use cases, sometines can increase the accuracy by 50~80\% accuracy. 

% As of now, developers mainly rely on manual prompting to optimization their applications. And we have quickly observed the limitation of the manual prompting:
% (1) it is time-consuming and labor-intensive as every time you switch to a new model, you have to start from scratch.
% (2) the manual prompting process itself is fraustrating as as of right now, LLMs continues to be sensitive to the tiny changes of words in the prompts~\cite{}, and there is no research indicates we can improve this.
% (3) as the LLM applications are getting more complex, it often become a complicated graph system, such as multi-hop RAG~\cite{khattab2022demonstrate} and Agent~\cite{yao2022react} making manual prompting infeasible.


\begin{remark}
    We need re-do the outline:

   
1. Introduction

Motivation, gap, significance 

Contribution bullets


2.Related Work

Summarize single-node prompt optimization vs. multi-node challenges

Position your method relative to these


3. Problem Formulation and Method

Define the multi-node LLM graph

Show how textual gradient backprop extends to functional nodes and cycles

Introduce “peer nodes,” “error-only gradient” strategy


4. Implementation Details (Optional or in Appendix)

AdalFlow specifics: Parameter structure, prompts, meta-prompts


5. Experiments

Research questions, datasets, baselines

Detailed results and ablation studies

Discussion of insights


6. Conclusion and Future Work

Recap main achievements

Limitations or open questions

Next directions

\end{remark}

\section{Introduction}

\paragraph{In-context learning revolutionized both AI and software development.}
The emerging in-context learning capabilities of Large Language Models (LLMs)~\cite{brown2020language} have revolutionized the fields of artificial intelligence and software development.
Both industry product teams and academic researchers are heavily invested in exploring and building applications powered by LLMs.
These applications, categorized into three primary types—chatbots~\cite{}, Retrieval-Augmented Generators (RAGs)\cite{khattab2022demonstrate}, and autonomous agents\cite{yao2022react,kimllm}—are poised to replace traditionally rule-based software systems, fundamentally transforming both the front-end and back-end of software architectures
The art of crafting prompts that can be effectively interpreted by LLMs has given rise to a new form of engineering, known as \textit{prompt engineering}\cite{wei2022chain,shinn2024reflexion},
for adapting pre-trained LLMs to downstream tasks.
This emerging field has been shown to significantly enhance performance,
with reported gains of up to $40\%$\cite{khattab2022demonstrate} in accuracy in certain scenarios.

\paragraph{Challenges in Manual Prompting.}
Modern Large Language Model (LLM) applications often comprise multiple interacting components—LLMs, retrievers, and functional
modules for data processing or formatting—leading to highly intricate AI systems.
Yet, most developers currently rely on \textit{manual prompting} to tailor their applications. While effective to some extent, this approach has several limitations:
\begin{enumerate}
    \item \textbf{Time-Consuming and Labor-Intensive:} Developers often have to start from scratch each time they switch to a new model, leading to inefficiencies.
    \item \textbf{Prompt Sensitivity:} LLMs remain highly sensitive to subtle changes in prompt wording~\cite{}, making manual optimization a frustrating and often unpredictable process. To date, no robust methods exist to address this sensitivity.
    \item \textbf{Complexity of Modern LLM Applications:} As LLM applications become more sophisticated, such as multi-hop RAG systems~\cite{khattab2022demonstrate} or agent-based architectures~\cite{yao2022react}, the manual prompting process becomes infeasible due to the intricate interdependencies and graph-like structures within these systems.
\end{enumerate}

\paragraph{Into Automatic Prompt Engineering (APE).}
To address these issues, we formalize \textbf{Automatic Prompt Engineering (APE)} as a process for automating manual prompt engineering.
Anything that enters an LLM as part of its input sequence can be \textit{engineered and optimized}, including task instructions, output formats, few-shot demonstrations,
retrieval context, tool usage seen in agents, and even special tokens.
While prior work proposes multiple terminologies for prompt engineering and APE (e.g., \cite{schulhoff2024prompt}), we aim for simplicity in describing the field.

Recent studies illustrate various ways LLMs themselves can be harnessed to automate prompt engineering.
For instance, LLM-based optimizers propose new prompts~\cite{yang2023large}, use textual auto-differentiation~\cite{pryzant2023automatic,yuksekgonul2024textgrad,wang2024correctly}
analog to the gradient descent in continous optimization~\cite{linnainmaa1970representation, linnainmaa1976taylor,beck2017first}
or leverage graph-based strategies~\cite{zhugegptswarm}. The prompts used by such ``optimizer'' LLMs are often referred to as ``meta-prompts''~\cite{zhou2022large}. Other approaches, such as RLPrompt~\cite{deng2022rlprompt} and Tempera~\cite{zhang2022tempera}, use reinforcement learning or small neural layers in tandem with a frozen LLM to adapt it for downstream tasks. All of these efforts underscore the growing variety of methods for \textit{automating prompt optimization}.

\paragraph{The Need for a Comprehensive Framework.}
Despite these advances, current methods largely address specific aspects of prompt design (e.g., optimizing the task instruction or few-shot demonstrations~\cite{khattab2022demonstrate}) and
often remain disconnected from more complex, multi-node LLM architectures.
To our knowledge, there is currently no unified system that allows developers to build and optimize \emph{any} LLM application in a single environment.
\emph{LLMDiff}, integrated within the AdalFlow library, will be the first auto-grad system offering this level of flexibility---much like how PyTorch~\cite{paszke2019pytorch} and
TensorFlow~\cite{abadi2016tensorflow} can automatically differentiate any combination of basic neural networks (e.g., RNNs, CNNs, Transformers).
By unifying automatic differentiation, prompt optimization, and multi-node support under one coherent framework, LLMDiff provides a powerful new paradigm for large-scale LLM development.

% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}[t]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{classification_training_map.png} % Replace with your first image file
%         \caption{\textbf{First Image Caption.} Description of the first image.}
%         \label{fig:sylph1}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{classification_opt_prompt.png} % Replace with your second image file
%         \caption{\textbf{Second Image Caption.} Description of the second image.}
%         \label{fig:sylph2}
%     \end{subfigure}
%     \caption{\textbf{The before and after of a prompt optimized in TextGrad2.0.} xxx}
%     \label{fig:sylph}
% \end{figure*}

\paragraph{Our Contributions: Auto-Optimizing Any LLM Application with \textit{LLMDiff} and \textit{AdalFlow}.}

First, to better understand the challenges that arise when attempting to \emph{auto-optimize} compound AI systems,
we introduce \emph{Automatic LLM Application Optimization (ALAO)}.
% Rather than proposing a definitive solution to these complexities, 
ALAO \textit{formulates} and \textit{defines} the scope of key issues in a rigorous mathematical manner and graph-based representation,
laying the groundwork for further research and system design.

Then, we present \textbf{LLMDiff}, which contributes four key innovations to the field of APE to enable fully automate any LLM applications:
\begin{itemize}
    \item \textbf{Multi-node Gradient Pass-Through:} As a compound LLM system can have multiple LLM nodes, with other interweaving components such as retrievers for context or other functional components
          (e.g., context deduplication in multi-hop RAGs~\cite{khattab2022demonstrate} or data formatting in agents~\cite{yao2022react}), we introduce a mechanism for passing gradients through purely these functional intermediate nodes.
    \item \textbf{Cyclic Structures:} Many systems, such as multi-hop RAGs~\cite{khattab2022demonstrate} or React Agent~\cite{yao2022react},
          contain loops in their execution flow. We propose a method to accumulate the gradients into the LLM optimizer properly,
          allowing the optimizer to be aware of how many times the LLM has been called due to the cycles, and have the gradient layed out in the order they are generated.

    \item \textbf{Peer Nodes:}
          (1) Subprompts (e.g., task instructions, output formats, few-shot examples) are modeled as separate \emph{peer nodes} instead of a single big prompt,
          to improve the effectiveness of the optimier and to counter-act the ``lost-in-the middile''~\cite{liu2024lost} effect.
          (2) To ensure that the \textit{backward engine} LLM can attribute the ``errors'' to the correct subprompt and for more token-efficient training,
          we propose a new gradient update method where the gradients to all precedessor nodes are computed in a single backward pass.
    \item \textbf{Selective Gradient Computation:} The optimizer can not learn ``specific errors'' from high-performaning samples other than being the turn to ``rephrase'' the existing prompt.
          As many LLM apps can start with decently high accuracy well above 60\%, the random batch training~\cite{pryzant2023automatic,yuksekgonul2024textgrad} will spend the majority of the tokens on
          samples without high-value training signals.
          We propose to only compute gradients for ``error'' samples, replacing the gradients for correct samples with one manual gradient as ``you are having a high accuracy''.
          This makes the training +60\% more token-efficient and faster compared with text-grad~\cite{pryzant2023automatic,yuksekgonul2024textgrad} with even higher accuracy by ``emphasizing''
          the most informative training signals.
\end{itemize}



\paragraph{Empirical Validation.}
Collectively, we refer to these advancements as \textbf{LLMDiff},
demonstrating significantly faster convergence rates and improved accuracy across a diverse range of applications, including single-node LLM classifier and question answering,
multi-node vanilla RAGs~\cite{lewis2020retrieval}, multi-hop RAGs~\cite{khattab2022demonstrate}(w/ or w/o cycles), and trainable ReAct agent~\cite{yao2022react}(w/ or w/o trainable LLMs for tool usage),
evaluated on various benchmarks.
Furthermore, we discover that
by integrating few-shot optimization seamlessly provided in \textit{AdalFlow}, our system surpasses existing approaches on final accuracy, inference speed, and no training cost by a large margin while maintaining scalability,
token efficiency at training time, and ease of use.






==> tex/methods.tex <==
\section{Methods}

We first formalize Automatic LLM Application Optimization (ALAO) and its subset, Automatic Prompt Engineering (APE) in  Section~\ref{sec:alao_ape}.
We then introduce the premilinary concept of textual auto-differentiation in Section~\ref{sec:interpreting_text_grad} by
clearly defining the graph with AdalFlow and explaining the key steps in the forward and backward pass in the training process.

Our contributions are two folds: A comphrensive approach on auto-differentiate any compound LLM system and a more efficient and effective training method.
We will introduce the Auto-differenate any compound LLM system in Section~\ref{sec:llm_diff} and the efficient training for textual auto-differentiation in Section~\ref{sec:token_efficient_text_grad}.
\textit{Note: To make the mathematical formulations more concrete, we draw the concepts from AdalFlow.}



\subsection{ALAO and APE} {\label{sec:alao_ape}}

\minisection{Automatic LLM Application Optimization (ALAO)} refers to the process of automatically optimizing a compound AI system that consists of
multiple LLMs, each designed for specific functionalities (e.g., routing~\cite{hu2024routerbench}, retrieval, generation),
by manipulating the prompt, the hyperparameters of each component, and even training/finetuning each LLM itself.
We have \textit{Automatic Prompt Engineering (APE)} as a subset of ALAO that focuses on optimizing the prompts of LLMs in a compound system, which
will be the main focus of this paper.

\minisection{Automatic prompt engineering (APE).}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\textwidth]{fig/multi_hop_rag_cycle_component.png}
    \caption{Cycles in a Multi-Hop RAG system. The sub query generator and sub query retriever are called twice in a for loop.}
    \label{fig:multi_hop_rag_cycle}
\end{figure}
Mathematically, we can formulate the APE problem as a graph optimization problem.
Let $\mathcal{G} = (\mathcal{N}, \mathcal{E})$ represent the LLM compound system as a \textit{directed graph} (possibly cyclic), where:
\begin{itemize}
    \item $\mathcal{N} = \{\mathcal{M}_i, \mathcal{R}_i, \dots\}$ represents component nodes (e.g., LLMs, retrievers) in the system.
    \item $\mathcal{E}$ represents directed edges defining the flow of data and dependencies between nodes, which may include cycles, such as in the case of Multi-hop RAG~\cite{khattab2022demonstrate} and ReACT agent~\cite{yao2022react} that require iterative processing or feedback mechanisms.
\end{itemize}

APE optimizes the prompts $\mathcal{P}_i$ for each LLM $\mathcal{M}_i$ within this graph, considering both system-level objectives and
sub-system-specific (sub-task) objectives, similar to multi-task learning in model training~\cite{phan2021cotext,li2021referring}.
We define a subset of components $\mathcal{N}_{T_{i}} \subseteq \mathcal{N}$ associated with each task $T_i$,
each with its own task-specific loss function $\mathcal{L}_{T_{i}}$.

For example, in the Multi-hop RAG system in Figure~\ref{fig:multi_hop_rag_cycle}, the system has two tasks: (1) a multi-hop retriever that consists of a sub-query generator and a sub-query retriever,
and (2) a generator that generates the final response.
Ideally, we want to optimize the whole system using two task-specific loss functions: one associated with metrics like Mean Reciprocal Rank (MRR) for the retriever so to train the ``query-generator''
and another associated with any generation metric like BLEU~\cite{papineni2002bleu}, BertScore~\cite{zhang2020bertscore}, or even LLM as a judge~\cite{zheng2023judging} for the final response generation.

Multi-task learning is important as LLM are natually strong few-shot learners~\cite{brown2020language} for any task such as retrievers and rerankers~\cite{qin2023large}, classifiers, and even generation tasks.
% \begin{enumerate}
%     \item For a retrieval task that has used LLM as a retriever and rerankers~\cite{qin2023large}, $\mathcal{L}_T$ might measure the quality of retrieved documents using metrics like mean reciprocal rank (MRR).
%     \item For a generation task, $\mathcal{L}_T$ is to measure ROUGE~\cite{}, BLEU~\cite{}, BertScore~\cite{}, or even LLM as a judge~\cite{} when the ground truth is not available.
%     \item For using LLM as classifier etc, $\mathcal{L}_T$ will be to measure the accuracy, F1 score, etc.
% \end{enumerate}


\begin{equation}\label{eq:multi_task_loss}
    \mathcal{L}(\mathcal{P}) \;=\; \bigcup_i \mathcal{L}_{T_{i}}(\mathcal{P}_{\mathcal{N}_{T_{i}}}), \\
    \mathcal{P}^* = \arg\min_{\mathcal{P}}  \bigcup_i \mathcal{L}_{T_{i}}(\mathcal{P}_{\mathcal{N}_{T_{i}}})s
\end{equation}
where $\bigcup_i$ denotes the union over all tasks in the system, and $\mathcal{P}_{\mathcal{N}_{T_{i}}}$ represents the trainable prompts of LLM components
in $\mathcal{N}_{T_i}$.
This generalizes APE to jointly optimize multiple prompts (or subprompts) across the entire system with respect to multiple tasks.

In LLM-Diff, each component is a \textit{GradComponent}, similar to PyTorch's \textit{Module}, that can be an LLM, a retriever, or any other operation.
AdalFlow allows you to draw a \textit{component graph} such as the one in Figure~\ref{fig:multi_hop_rag_cycle}.




\subsection{Interpreting Textual Auto-differentiation with AdalFlow}{\label{sec:interpreting_text_grad}}



\minisection{Defining the dynamic computation graph $\mathcal{G}_{p}$.} In PyTorch~\cite{paszke2019pytorch}, weights are defined as `Parameter' and inputs and outputs are defined as `Tensor'.
Each type of layer is named as a `Module'. In AdalFlow, our main goal is to optimize the prompt $\mathcal{P}_i$ of each LLM $\mathcal{M}_i$ in the graph $\mathcal{G}$.
According to the LLM application patterns mentioned in Section~\ref{prompt_engineering}, the prompt $\mathcal{P}_i$ can be a combination of
task instructions, few-shot demonstrations, output format, and tools.
To auto-optimize this graph, we need to trace the inputs, input arguments and outputs of each component in the graph $\mathcal{G}$
which potentially has cycles as shown in Figure~\ref{fig:multi_hop_rag_cycle}
, and the dependencies between them.
We use \textit{Parameter} to represent these inputs and outputs, and these parameters will form a dynamic parameter computation graph $\mathcal{G}_{p}$
which is Directed Acyclic Graph (DAG) at runtime, where the nodes are the parameters and the edges are the dependencies between them.
% todo: make this graph more presentable, with better explanation
In AdalFlow, each ``Parameter'' is assigned to one of 5 types:
\begin{enumerate}
    \item \textbf{PROMPT} for task instruction, output format, tool use, etc.
    \item \textbf{DEMOs} for few-shot demonstrations that often sampled from the training set, thus differs from how the `Prompt' type is trained.
    \item \textbf{INPUT} for component inputs
    \item \textbf{OUTPUT} for component's output parameter.
          Each node/Component has and only has one output parameter.
          In AdalFlow, the output value is saved at the \textit{data} field of the output parameter as a structure of \textit{GeneratorOutput} for one basic LLM call or
          \textit{RetrieverOutput} for one retriever call.
    \item \textbf{HYPERPARAM} for this node's hyperparameters such as the `top-k' for the retriever.
\end{enumerate}
Now, the dynamic computation graph $\mathcal{G}_{p}$ = $(\mathcal{N}_p, \mathcal{E}_p)$ with $v$ denotes each vertice is defined as follows:
\begin{equation}
    \label{eq:forward_pass}
    v = f_c\big(\text{PredecessorsOf}(v)\big), \quad \text{for each } c \in \mathcal{N} \text{ in graph } G.
\end{equation}
where $f_c$ is the component($c$)'s transformation function,
$\text{PredecessorsOf}(v)$ refers to the input arguments for this node represented as parameters of five types in $\mathcal{G}_{p}$.
, and $v$ is the output parameter of this node.
% TODO: add the multi-hop RAG figure


\minisection{Textual Backpropagation for LLMs}
\paragraph{1. Forward Pass.} The forward pass computes the output of each node (component) $v \in \mathcal{N}$
from $\mathcal{G}$ using Eq.~\ref{eq:forward_pass}, forming the runtime dynamic computation graph.

\paragraph{2. Textual Loss Definition.}
The downstream loss $\mathcal{L}$ is defined over one or more target components,
each with its own specific task and each evaluated on its own metric
$s_v$ from evaluation function $e_v$, with the textual description of the evaluation function $\text{e}_{\text{desc},v}$ in the graph.
This loss for one ending component can be specified using unstructured natural language via LLMs,
where you can think of the loss as a textual objective function for the LLM to optimize:
\begin{subequations}
    \begin{align}
        s_v         & = e_v(v, v_{gt}), \quad s_v \in [0, 1] \quad \text{or} \quad s_v \in \mathbb{R},
        \\
        \mathcal{L} & = \bigl(\text{e}_{\text{desc},v},\, v, v_{gt}, \, s_v\bigr),
    \end{align}
\end{subequations}
where $v$ is usually the final output parameter in $\mathcal{G}_{p}$, and $v_{gt}$ is the ground truth value for $v$ which is optional if LLM as a judge~\cite{zheng2023judging} is used.
See \textit{EvalFnToTextLoss} in AdalFlow for the implementation of this loss component.
It creates an output parameter of type \textit{LOSS\_OUTPUT} to track \( s_v \).
In AdalFlow, we use the following a combination of two templates to define the loss(aka textual objective function) which is formed with Jinja2~\footnote{\url{https://jinja.palletsprojects.com/en/stable/}}
templates where inputs include the $v$ and $v_{gt}$,  and the $e_{\text{desc},v}$ and $s_v$ are all presented in this prompt as a form of textual loss to the ``backward engine'' LLM.
\begin{lstlisting}[
    basicstyle=\ttfamily\small,
    breaklines=true,
    language=Python,
    keywordstyle=\color{blue}\bfseries,
    stringstyle=\color{orange},
    commentstyle=\color{green!50!black},
    frame=single,
    showstringspaces=false,
    tabsize=4,
    numbers=left,
    numberstyle=\tiny\color{gray}
]
LOSS_CONVERSATION_TEMPLATE_STRING = r"""
The variable is passed to the eval function and compared with a target/ground truth value.

EVAL_FUNC: {{eval_fn_desc}}

INPUTS:
{% for key, (value, eval_type) in inputs.items() %}
({{ key }}) (role: {{ value.role_desc }}),
data: {{ value.prompt_data }},
input_to_eval_fn: {{ value.eval_input }},
data_type: {{ eval_type }}
{% endfor %}

OUTPUTS/SCORE: {{response_value}}
{% if metadata %}
Note: {{metadata}}
{% endif %}"""

OBJECTIVE_INSTRUCTION_BASE = r"""<OBJECTIVE_FUNCTION>
Your task is to provide the response with specific feedback based on the ground truth and the score in the "<OUTPUTS/SCORE>".
Especially when the score is low.
Be CONCISE.
Be specific on why it has a low score.
e.g. "The retrieved context is not enough to answer the question so the problem relies on the retrieval part."
</OBJECTIVE_FUNCTION>"""
\end{lstlisting}

\paragraph{3. Backward Pass (Textual Gradients).}
Once the forward pass and loss evaluation have been completed,
the system computes textual gradients that flow backward through the \textit{dynamic computation graph} $\mathcal{G}_{p}$.


\subparagraph{Computing the gradient for the final output node inside of the LossComponent.}
% Consider the final node $(v_o \in \mathcal{N})$ in $\mathcal{G}$,
% which typically is an LLM call generating the final system response and whose output is directly pass to a loss component which generates the loss as in Eq.~\ref{eq:final_node_gradient}.
As this final output node has only one successor which is the loss component,
its gradient is computed in the loss component’s backward pass as follows:
\begin{equation}\label{eq:final_node_gradient}
    \frac{\partial \mathcal{L}}{\partial v_o}
    \;=\;
    \text{LLM}_{\text{backward}}\bigl(\mathcal{L}\bigr),
\end{equation}
where the loss $\mathcal{L}$ is passed to the frozen backward engine LLM which will be referred to as the \textit{backward engine} from here on to generate the textual gradients.


\subparagraph{Computing the gradients for intermediate LLM nodes inside of the Generator.}

For an intermediate node \(v \in \mathcal{N}\), let \(\mathrm{SuccessorsOf}(v)\) be the set of its successors.
The textual gradients \(\frac{\partial \mathcal{L}}{\partial v}\)
are aggregated from the feedback from each successor \(w\):
\begin{equation}\label{eq:intermediate_grad}
    \frac{\partial \mathcal{L}}{\partial v}
    \;=\;
    \bigcup_{w \in \mathrm{SuccessorsOf}(v)} \text{LLM}_{\text{backward}}\bigl(v,\; w,\; \tfrac{\partial \mathcal{L}}{\partial w}\bigr),
\end{equation}
where these following texts are formed into a prompt context for the backward engine:
% \begin{equation}\label{eq:grad_f_definition}
%     \nabla f(w,\; v,\; \cdot)
%     \;=\;
%     \text{LLM}_{\text{backward}}\Bigl(w \;\oplus\; v \;\oplus\; \text{Feedback}\bigl(w,\; \cdot\bigr)\Bigr).
% \end{equation}
% Here, \(\nabla f\) invokes the backward engine to produce textual feedback for \(v\) based on
(i) the successor node \(w\),
(ii) the gradient of the successor node \(\tfrac{\partial \mathcal{L}}{\partial w}\), and
(iii) any contextual information needed to interpret how \(v\) influences \(w\).
This means that any intermediate node \(v\) will receive \(\bigl|\mathrm{SuccessorsOf}(v)\bigr|\) gradients, one from each of its successors.

If our LLM application has only one LLM call(a ``Generator''), then $\frac{\partial \mathcal{L}}{\partial v_o}$ is the gradient attached to the output prameter,
and $\frac{\partial \mathcal{L}}{\partial v}$ can be the gradient attached to prompt parameter and the $\frac{\partial \mathcal{L}}{\partial w } = \frac{\partial \mathcal{L}}{\partial v_o}$.

Here is the template for combing $\bigl(v,\; w,\; \tfrac{\partial \mathcal{L}}{\partial w}\bigr)$:
\begin{lstlisting}[
    basicstyle=\ttfamily\small,
    breaklines=true,
    language=Python,
    keywordstyle=\color{blue}\bfseries,
    stringstyle=\color{orange},
    commentstyle=\color{green!50!black},
    frame=single,
    showstringspaces=false,
    tabsize=4,
    numbers=left,
    numberstyle=\tiny\color{gray}
]
CONVERSATION_START_INSTRUCTION_CHAIN = r"""
{{variable_and_peers_info}}

Here is a conversation with the language model (LM):
{{conversation_str}}
"""

# For the generator in the chain,
OBJECTIVE_INSTRUCTION_CHAIN = r"""
This conversation is part of a larger system. The <LM_OUTPUT> was later used as {{response_desc}}.
<OBJECTIVE_FUNCTION>
Your goal is to give feedback to the variable to guide the LLM_OUTPUT according to feedback: {{response_gradient}}
{% if instruction_to_backward_engine %}
Note: {{instruction_to_backward_engine}}
{% endif %}
</OBJECTIVE_FUNCTION>"""

OBJECTIVE_INSTRUCTION_CHAIN = r"""
This conversation is part of a larger system. The <LM_OUTPUT> was later used as {{response_desc}}.
<OBJECTIVE_FUNCTION>
Your goal is to give feedback to the variable to guide the LLM_OUTPUT according to feedback: {{response_gradient}}
{% if instruction_to_backward_engine %}
Note: {{instruction_to_backward_engine}}
{% endif %}
</OBJECTIVE_FUNCTION>"""

LLM_CONVERSATION_TEMPLATE = r"""
LM_INPUT: {{input_value}}
LM_OUTPUT: {{llm_output}}"""
\end{lstlisting}
The Meta-prompt template for the backward engine used in loss component and a generator component along with other essential data structures are provided
in Section~\ref{appendix: meta_prompts_backward_engine}.

% todo: move all of this in the appendix


\paragraph{4. Update Step (Textual Gradient Descent).}
Once the textual gradients \(\tfrac{\partial \mathcal{L}}{\partial v}\) are
computed for all parameters(only for those that require gradients),
the system performs a \emph{Textual Gradient Descent (TGD)}
step to update the prompt parameters \(\mathcal{P}_v\):

\begin{equation}
    \label{eq:textual_update_step}
    \mathcal{P}_{v_{\text{new}}}
    \;=\;
    \text{LLM}_{\text{opt}}\Bigl(v, \text{GradientContext}(v), \tfrac{\partial \mathcal{L}}{\partial v}\Bigr).
\end{equation}

where \(\text{GradientContext}(v)\) includes input arguments, output collected in the forward pass and $s_v$ from the backward pass,
and \(\text{LLM}_{\text{opt}}\) is the optimizer LLM that generates the updated prompt $\mathcal{P}_{v_{\text{new}}}$.


\paragraph{Minibatch Training.}
Text-Grad~\cite{yuksekgonul2024textgrad} trains the system with standard minibatch training using three splits of the dataset:
$\mathcal{D}_{\text{train}} = \{(x_i, y_i)\}$ for loss and gradient computation,
$\mathcal{D}_{\text{validate}}$  for validating propmpt updates,
and $\mathcal{D}_{\text{test}}$ for final evaluation.
During training, data from $\mathcal{D}_{\text{train}}$ is processed in minibatches of size $B = 4$ in LLMDiff ($3$ in Text-Grad).
For each minibatch $\{(x_i, y_i)\}_{i=1}^B$, the forward pass computes predictions $\{\hat{y}_i\}_{i=1}^B$ through the graph $\mathcal{G}$.
In Text-Grad~\cite{yuksekgonul2024textgrad}, the batch loss $\mathcal{L}_{\text{batch}}$ is computed by backpropagate each sample in the batch:

\begin{equation}
    \mathcal{L}_{\text{batch}} = \frac{1}{B} \sum_{i=1}^B \mathcal{L}(y_i, \hat{y}_i),
\end{equation}

where \(\mathcal{L}(y_i, \hat{y}_i)\) is the loss for a single sample \(i\).
For each training step, the validation accuracy is computed on $\mathcal{D}_{\text{validate}}$
to evaluate the new prompts.
If the performance is improved, the prompts are updated.
If not, the prompts are rejected and the previous prompts are used for the next training step.
The final test accuracy is computed on $\mathcal{D}_{\text{test}}$ to evaluate the final system's performance.

\subsection{Auto-differentiate Any Compound LLM System}{\label{sec:llm_diff}}
We will introduce how LLM-Diff advance the Textual Auto-differentiation to any compound LLM System that can (1) have multiple LLM calls,
(2) interweave other components like retrievers, or any other functional code connecting in between, (3) have cycles by calling certain components multiple times in a single system.
This has resulted to the updates of the backward pass from the initial Eq.~\ref{eq:intermediate_grad} to Eq.~\ref{eq:intermediate_grad_functional}, and to Eq.~\ref{eq:cyclic_grad_call}.


\minisection{Multi-nodes} {\label{sec:multi_node_text_grad}}

\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{fig/multi_hop_rag_comp_graph.png}
    \caption{The runtime dynamic computation graph $\mathcal{G}_{p}$ for Multi-hop RAG with a cyclic structure.
        We have added a deduplication component to deduplicate the retrieved documents from two retrievers.}
    \label{fig:multi_node_text_grad}
\end{figure}

% file:///Users/liyin/.adalflow/ckpt/MultiHopRAGCycleAdal/debug_text_grads/trace_graph_sum_id_6eacab1c-1ed7-44ec-8b23-3183396392d3_interactive_graph.html

To build a compound LLM system (e.g., involving multiple \textit{Generators}), additional intermediate components may be required.
For instance, Figure~\ref{fig:multi_node_text_grad} shows a \textit{Deduplication} node that merges two lists of retrieved documents in a multi-hop RAG~\cite{khattab2022demonstrate}.
Such a node often does not involve any AI module and therefore does not introduce any trainable parameters; rather, it simply performs data manipulation.

\paragraph{Gradient Pass-Through for Functional Nodes.}
Let \(v \in \mathcal{N}_p\) be a purely functional node as seen in the example,
\begin{equation}
    v = f_v(L_1, L_2) \;=\; \text{Deduplicate}(L_1 \cup L_2),
\end{equation}
where \(L_1\) and \(L_2\) are outputs from previous \textit{Retriever} nodes.
Since \(v\) has no trainable parameters,
the gradient from \(v\) is simply passed backward to its predecessors \(L_1\) and \(L_2\).

To write it formally, let \(\mathrm{PredecessorsOf}(v)\) be the set of predecessors of \(v\),
we can rewrite its gradient computation as:
\begin{equation}
    \label{eq:intermediate_grad_functional}
    \frac{\partial \mathcal{L}}{\partial v}
    \;=\;
    \bigcup_{w \in \mathrm{SuccessorsOf}(v)}
    \begin{cases}
        \tfrac{\partial \mathcal{L}}{\partial w},                                                   & \text{if } w  \text{ is a functional node output}, \\[6pt]
        \text{LLM}_{\text{backward}}\bigl(v,\; w,\; \tfrac{\partial \mathcal{L}}{\partial w}\bigr), & \text{otherwise}.
    \end{cases}
\end{equation}
These gradients are then routed directly to \(L_1\) and \(L_2\). This mechanism preserves the chain rule~\cite{linnainmaa1970representation,linnainmaa1976taylor,beck2017first} across the entire graph~\(\mathcal{G}\),
ensuring end-to-end optimization in a multi-node LLM application.
Therefore, LLM-Diff has modified the backward pass from Eq.~\ref{eq:intermediate_grad} to Eq.~\ref{eq:intermediate_grad_functional}.

\paragraph{Handling Duplicate Gradients in Multi-node Systems.}
In a multi-node setup, a single parameter node may receive
repeated pass-through gradients as a result of having multiple successors which can receive the same pass-through gradients,
causing duplicate gradients for a single parameter.
To mitigate this, we store each gradient in a hash-based data structure (e.g., a \texttt{set} or a dictionary keyed by a unique gradient identifier).
Specifically, each gradient entry includes contextual information such as the data ID,
call index \(t\), and textual gradient content.
By hashing these entries and inserting them into a set,
the system automatically merges duplicate gradients,
preventing an unbounded accumulation of identical gradient.
% This approach ensures that each unique gradient is processed exactly once while preserving the correct ordering for time-sequential feedback in cyclic structures.








\minisection{Cycles}
\label{sec:cyclic_structures}

Certain LLM applications (e.g., multi-hop RAG~\cite{khattab2022demonstrate},
iterative ReACT agents~\cite{yao2022react}) involve cycles in the component graph \(\mathcal{G}\).
In these scenarios, an LLM node may be invoked multiple times in a
single forward pass, accumulating multiple gradients in the backward
pass. To handle these cases, we maintain a distinct ordering of gradients, tied to the call index of each LLM invocation, rather than simply merging them into a single aggregated gradient.

\paragraph{Time-sequential Gradients for Cyclic Structures}

Formally, let \(c\) be a node in \(\mathcal{G}\) that is called \(T_c\) times during a single runtime for
one data sample.
For every call index \(t \in \{1, \ldots, T_c\}\),
the gradient obtrained from the \(t\)-th invocation is denoted as
\(\tfrac{\partial \mathcal{L}}{\partial v^{(t)}}\) where \(v^{(t)}\) is the output of the \(t\)-th call.
For the trainable precedessor parameters of \(c\), the gradients are aggregated as:
% \begin{equation}\label{eq:cyclic_grad_call}
%     \frac{\partial \mathcal{L}}{\partial P_c}
%     \;=\;
%     \bigcup_{t=1}^{T_v}
%     \left\{
%     \Bigl(t,\;\tfrac{\partial \mathcal{L}}{\partial v^{(t)}}\Bigr)
%     \right\}.
% \end{equation}
\begin{equation}\label{eq:cyclic_grad_call}
    \frac{\partial \mathcal{L}}{\partial P_c}
    \;=\;
    \bigcup_{t=1}^{T_v}
    \left\{
    \Bigl(
    t,\;
    \frac{\partial \mathcal{L}}{\partial v^{(t)}}
    \;\cdot\;
    \frac{\partial v^{(t)}}{\partial P_c}
    \Bigr)
    \right\}.
\end{equation}
Here, each tuple $\Bigl(
    t,\;
    \frac{\partial \mathcal{L}}{\partial v^{(t)}}
    \;\cdot\;
    \frac{\partial v^{(t)}}{\partial P_c}
    \Bigr)$
captures both the call index \(t\) and the corresponding gradient, enabling the backward engine to preserve the temporal or iterative sequence in which the calls were made.

\paragraph{Implementation}

If there is only one data point in the minibatch, the gradients can be appended to a single list in the correct order. However, in practice, the system may process multiple data points simultaneously; thus, each gradient tuple must also record the data index (or ID) to accurately track the calling order for each sample. By storing both the call index \(t\) and the data ID, the backward pass faithfully reproduces the chain rule across multiple invocations of the same LLM node, preserving end-to-end differentiability in cyclic LLM applications.


\paragraph{Meta-prompt Template for Cyclic Structures}
Second, we add the following prompt to inform the optimizer LLM and the backward engine.
\begin{lstlisting}
If the same DataID has multiple gradients, it means this component/variable is called multiple times in the compound system(with a cycle) in the same order as it appears in the gradient list.
\end{lstlisting}


% Please refer to AdalFlow~\cite{} for the detailed implementation of each component to form a compound AI system that is auto-differentiable.
\subsection{Efficient Training method for Textual Auto-differentiation}
{\label{sec:token_efficient_text_grad}}

Next, we will improve the training efficiency and effectiveness by (1)
introducing  the concept of peers where we compute all the gradients for the peers(precedessors) of a node in parallel, (2)computing gradients only for high-performing training samples,
and (3) introducing mini-batch validation and generating and validating multiple new prompts proposals for the same backward pass.
Compared with standard textual auto-differentiation, LLM-Diff is 3X faster when searching through the same size of space(the same number of prompts).

\minisection{Peers} {\label{sec:peer_nodes}}
First, complex LLM prompts typically include distinct subprompts (e.g., task instructions, few-shot examples, output formatting).
Allowing each of these subprompt to be its own parameter node in the graph $\mathcal{G}_{p}$ can better optimize each part without overwhelming the optimizer with a complicated prompt.
And this optimization work out of the box within Text-Grad.

However, we find out when multiple parameters are used, there can be \textbf{cross-contamination} between the parameters.
That is the LLM optimizer can propose a task instruction with few-shot examples or output format, this cross-contamination can lead to a human-uninterpretable prompt and be suboptimal in performance too.

Second, for complicated system like Multi-hop RAG, it is important for the last LLM which combines retrieved context from the multiple retrievers and the question for a final response
to know if the problem is on the context or on the prompt task instruction.

To prevent cross-contamination and to compute gradients more effectively and efficiently for these \textbf{peer nodes},

we introduce \textbf{Peer Nodes} in the computation graph $\mathcal{G}_{p}$.


The output $v$ is computed as a function of its peer predecessors:
\begin{equation}
    v = c_v(p_1, p_2, \dots, p_k),
\end{equation}
where $c_v$ represents the computational function of $v$.
Each $p_i$ can be one of the following types:
\begin{equation}
    P_v = \{P_v{\text{task}}, P_v{\text{few-shot}}, P_v{\text{out-format}}, \dots\}
\end{equation}

For each peer node $p_i$, the gradient of the loss $\mathcal{L}_v$ is computed jointly as:
\begin{equation}
    \left\{\frac{\partial \mathcal{L}_v}{\partial p_1}, \frac{\partial \mathcal{L}_v}{\partial p_2}, \dots, \frac{\partial \mathcal{L}_v}{\partial p_k}\right\}
    = \nabla f(v, \left\{ p_1, p_2, \dots, p_k\right\}, \frac{\partial \mathcal{L}_v}{\partial v}),
\end{equation}
where $\nabla f(...)$ generates the textual gradient for all peer nodes $p_i$ based on the feedback from $\mathcal{L}_v$.



\paragraph{Meta-prompt Template for Peer Nodes}
We add one instruction besides of the context of other peer info in the gradient prompt:
\begin{lstlisting}
    3. Consider the variable in the context of its peers if provided.
\end{lstlisting}
${v_{\text{sub}}}$ is represented as a prompt template used in both the backward engine and the optimizer.
\begin{lstlisting}
    VARIABLE_AND_PEERS_INFO = r"""
    <START_OF_VARIABLE_DESC>
    {{variable.name}}
    <TYPE> {{variable.param_type}} </TYPE>
    <ROLE> {{variable.role_desc}} </ROLE>
    <VARIABLE> {{variable.data}} </VARIABLE>
    <END_OF_VARIABLE_DESC>
    {% if peers %}
    <VARIBLE_PEERS>
    The variable is used together with the these peer variables to instruct the language model:
    {% for peer in peers %}
    {{loop.index}}.
    PEER_NAME: {{peer.name}},
    PEER_TYPE: {{peer.param_type}},
    PEER_ROLE: {{peer.role_desc}}
    WILL_BE_OPTIMIZED: {{peer.requires_opt}}
    {% if peer.data %}
    PEER_VARIABLE: {{peer.data}}
    {% else %}
    PEER_VARIABLE: EMPTY
    {% endif %}
    {% endfor %}
    </VARIBLE_PEERS>
    {% endif %}
    """
\end{lstlisting}

With this context, the optimizer will know to optimize each node in the peer sets separately.


\minisection{Loss and Gradients only for Error Samples}~\label{sec:loss_error_samples}


In numerical optimization, gradient descent is driven by the accumulated loss over all samples.
The larger the error on an example, the larger the contribution to the gradients.
However, in LLM based optimizers, for high-performing examples, it takes the same amount of `GradientContext' and `Feedback'.
We argue the positive `feedback` is not giving the optimizer valuable information to "correct" the prompt, but just letting the optimizer do more rephrasing on the existing prompt.
\[
    P(\text{No errors in batch}) = \frac{\binom{N_1}{n} \cdot \binom{N_0}{0}}{\binom{N}{n}}
\]

where:
\begin{itemize}
    \item \( N \) = Total samples = 50
    \item \( N_1 = 50 \cdot \text{Accuracy} \)
    \item \( N_0 = 50 \cdot (1 - \text{Accuracy}) \)
    \item \( n \) = Batch size = 4
\end{itemize}

For datasets starting at 50\% and 80\% accuracy:

\[
    P_{50\%} = \frac{\binom{25}{4} \cdot \binom{25}{0}}{\binom{50}{4}} = 0.0549 \, (5.49\%)
\]

\[
    P_{80\%} = \frac{\binom{40}{4} \cdot \binom{10}{0}}{\binom{50}{4}} = 0.3968 \, (39.68\%)
\]

This highlights the impact of dataset quality on optimization performance.

This takes extra tokens in the prompt, and due to the ``lost in the middle"~\cite{liu2024lost} effect, these correct
training samples in a minibatch end up more like a ``noise" to the optimization process rather than a useful signal.

Therefore, we proposed to only compute the gradients and loss for samples with an accuracy score lower than a threhold $\tau$.
\begin{equation}
    \mathcal{L} = \sum_{i=1}^B \mathcal{L}(y_i, \hat{y}_i) \quad \text{if} \quad s_i(y_i, \hat{y}_i) < \tau,
\end{equation}

Here are the benefits of this approach:
\begin{enumerate}
    \item \textbf{Speed and token-efficiency:} Assuming $n_e$ samples in a training set of size $n$, the loss is computed only for the $n_e$ samples with errors:
          At each step, the training is $\frac{n-n_e}{n}$ faster in converging and more token-efficient.
    \item \textbf{Better accuracy:} From our ablation study, we found that the accuracy is improved by X\%.
\end{enumerate}



\paragraph{LLMDiff Algorithm Implementation}

To manage repeated or duplicate gradient signals in a multi-node system, we can represent the unique gradient contributions as elements in a set. Let \(\mathcal{D}\) be the set of data indices, and let each parameter \(p_c\) collect gradients from \(\lvert \mathcal{D} \rvert\) data points. If a node \(v\) is invoked \(T_c\) times per data sample, the unique gradient set for parameter \(p_c\) can be written as:
\begin{equation}\label{eq:hash_grad_set}
    \mathrm{GradSet}(p_c)
    \;=\;
    \mathrm{Unique}\!\Biggl(\;
    \bigcup_{d \,\in\, \mathcal{D}}
    \bigcup_{t=1}^{T_c}
    \Bigl\{\,
    \bigl(d,\,t,\,
        \tfrac{\partial \mathcal{L}_d}{\partial v^{(t)}} \,\cdot\,
        \tfrac{\partial v^{(t)}}{\partial p_c}\bigr)
    \Bigr\}
    \Biggr),
\end{equation}
where:
\begin{itemize}
    \item \(d\) is the data index (e.g., an identifier for a sample in the minibatch).
    \item \(t\) is the call index (i.e., the \(t\)-th time node \(v\) is invoked).
    \item \(\tfrac{\partial \mathcal{L}_d}{\partial v^{(t)}}\) is the gradient of the loss for data point \(d\) w.r.t.\ the \(t\)-th output of node \(v\).
    \item \(\tfrac{\partial v^{(t)}}{\partial p_c}\) captures how the \(t\)-th invocation of \(v\) depends on parameter \(p_c\).
    \item \(\mathrm{Unique}(\cdot)\) (or equivalently a hash set) merges any duplicate gradient tuples to avoid counting them multiple times.
\end{itemize}
By storing each gradient entry \(\bigl(d,\,t,\,\cdot\bigr)\) in a hash-based data structure, the backward pass ensures that each unique gradient is accounted for exactly once,
preserving correct ordering and preventing the accumulation of duplicate gradients in the multi-node system.


\minisection{Mini-batch Validation and Multiple Prompt Proposals}~\label{sec:mini_batch_validation}

TODO: add back a simple version of the previous algorithm
\subsection{Integration of Few-Shot Learning}

Few-shot learning is seamlessly integrated as a subset of the APE framework. Demonstrations are treated as another form of Peer Nodes \( P_{\text{few-shot}} \), allowing automatic selection and optimization of examples from the training set.

\paragraph{Few-Shot Demonstration Selection}
Given a training set \( D \), candidate subsets are sampled and evaluated:
\[
    P_{\text{few-shot}} = \operatorname*{arg\,max}_{S \subset D} \text{Accuracy}(S)
\]
Demonstrations are validated using the same multi-stage process outlined in Section 3.3.

\paragraph{Adaptive Few-Shot Integration}
Demonstrations are optimized alongside other prompt components, ensuring alignment with task-specific objectives.

By combining these methodologies, \textbf{TextGrad 2.0} provides a unified and extensible framework for optimizing any LLM application efficiently and effectively.


% todo: extend to multi-task optimization


==> tex/related.tex <==
\vspace{-2mm}
\section{Related Work}
\vspace{-2mm}

As a paper to cover all existing LLM application patterns, from Chatbots, RAGs, to agents, and to automate prompt optimizing the LLM calls in these applications, leveraging the most effective and systematic approach, the related work is extensive. Instead of covering all papers, we would like to select the highlights of each category and to summarize the related work to reflect the whole prompt engineering as a whole.

\subsection{Prompt Engineering} \label{prompt_engineering}
The prompt engineering field can be mostly captured in the following 4 points:
\begin{enumerate}
    \item  In-context learning~\cite{brown2020language} is LLM’s ability to learn via the input sequence, it includes zero-shot and few-shot learning.
    \item RAG~\cite{lewis2020retrieval} adds new “knowledge” in the context and lowers “hallucination”
    \item CoT(aka “Let’s think step-by-step”)~\cite{wei2022chain} lets LLM generate more “reasoning” tokens to better elicit the right “answer”
    \item Agent~\cite{yao2022react, shinn2024reflexion} emphasizes the use of “tool” and the feedback from the tool for a “multi-step task”
\end{enumerate}

\minisection{Auto-Prompt Engineering}
So far, we observed three categories of auto-prompt engieering:
\begin{enumerate}
    \item Given a starter prompt, an LLM is programmed with prompt engineer personas ~\cite{} to generate various of new prompts that might work better for developers. This includes both the research such as OPRO~\cite{brown2020language} and the industry such as Anthropic\footnote{\url{https://docs.anthropic.com/en/docs/build-with-claude/prompt-engineering/prompt-improver}} will instruct the optimizer, which is likely an agent to check the existing prompt on multiple prompt engineering techniques and requirements to propose a final version.
    \item Text-Grad which uses a more systematic aproach analogous to the gradient descent in the continous optimization where both building the LLM applications, evaluating, and optimizing are all in the same place, similar to ai modeling is a way more systematic and prompising approach to prompt optimization.
    \item Automatically sample and validate the few-shot demonstrations from a training set ~\cite{} is another subset of the auto-prompt engineering, where the few-shot demonstrations are automatically sampled and validated to be used in the LLM applications.
\end{enumerate}

\paragraph{In-context learning revolutionized both AI and software development.}
The emerging in-context learning capabilities of Large Language Models (LLMs)~\cite{brown2020language} have revolutionized the fields of artificial intelligence and software development.
Both industry product teams and academic researchers are heavily invested in exploring and building applications powered by LLMs.
These applications, categorized into three primary types—chatbots~\cite{}, Retrieval-Augmented Generators (RAGs)\cite{khattab2022demonstrate}, and autonomous agents\cite{yao2022react,kimllm}—are poised to replace traditionally rule-based software systems, fundamentally transforming both the front-end and back-end of software architectures
The art of crafting prompts that can be effectively interpreted by LLMs has given rise to a new form of engineering, known as \textit{prompt engineering}\cite{wei2022chain,shinn2024reflexion},
for adapting pre-trained LLMs to downstream tasks.
This emerging field has been shown to significantly enhance performance,
with reported gains of up to $40\%$\cite{khattab2022demonstrate} in accuracy in certain scenarios.

\minisection{Automating LLM applications via both model finetuning and prompt optimization}
An LLM application is a compound AI system, and it can be further viewed in combination of model-training, hyperparameter optimization, and auto-prompt optimization.
~\cite{soylu2024fine} is the first that has optimized an AI system combining both model finetuning such as SFT and DPO with few-shot learning.
\minisection{Soft prompting}
[needs rewrite this section, this is just notes for soft prompting]
tuning soft prompts (e.g.,embeddings) which fall short of interpretabil-ity, reusability across LMs, and applicabilitywhen gradients are not accessible~\cite{deng2022rlprompt}
% TODO: add the data flow in the LLM applications in the appendix or related work


\paragraph{Challenges in Manual Prompting.}
Modern Large Language Model (LLM) applications often comprise multiple interacting components—LLMs, retrievers, and functional
modules for data processing or formatting—leading to highly intricate AI systems.
Yet, most developers currently rely on \textit{manual prompting} to tailor their applications. While effective to some extent, this approach has several limitations:
\begin{enumerate}
      \item \textbf{Time-Consuming and Labor-Intensive:} Developers often have to start from scratch each time they switch to a new model, leading to inefficiencies.
      \item \textbf{Prompt Sensitivity:} LLMs remain highly sensitive to subtle changes in prompt wording~\cite{}, making manual optimization a frustrating and often unpredictable process. To date, no robust methods exist to address this sensitivity.
      \item \textbf{Complexity of Modern LLM Applications:} As LLM applications become more sophisticated, such as multi-hop RAG systems~\cite{khattab2022demonstrate} or agent-based architectures~\cite{yao2022react}, the manual prompting process becomes infeasible due to the intricate interdependencies and graph-like structures within these systems.
\end{enumerate}

\paragraph{Automatic Prompt Engineering (APE).}
To address these issues, we formalize \textbf{Automatic Prompt Engineering (APE)} as a process for automating manual prompt engineering.
Anything that enters an LLM as part of its input sequence can be \textit{engineered and optimized}, including task instructions, output formats, few-shot demonstrations,
retrieval context, tool usage seen in agents, and even special tokens.
While prior work proposes multiple terminologies for prompt engineering and APE (e.g., \cite{schulhoff2024prompt}), we aim for simplicity in describing the field.

Recent studies illustrate various ways LLMs themselves can be harnessed to automate prompt engineering.
For instance, LLM-based optimizers propose new prompts OPRO~\cite{yang2023large}, use textual auto-differentiation~\cite{pryzant2023automatic,yuksekgonul2024textgrad,wang2024correctly}
analog to the gradient descent in continous optimization~\cite{linnainmaa1970representation, linnainmaa1976taylor,beck2017first},
few-shot learning with teacher reasoning~\cite{khattab2022demonstrate}, combines both instruction tuning and demonstration in MIPRO~\cite{opsahl2024optimizing},
or leverage graph-based strategies~\cite{zhugegptswarm}. The prompts used by such ``optimizer'' LLMs are often referred to as ``meta-prompts'' in APE~\cite{zhou2022large}. Other approaches, such as RLPrompt~\cite{deng2022rlprompt} and Tempera~\cite{zhang2022tempera}, use reinforcement learning or small neural layers in tandem with a frozen LLM to adapt it for downstream tasks. All of these efforts underscore the growing variety of methods for \textit{automating prompt optimization}.

(here, we miss a paragraph discussing single-node prompt optimization vs. multi-node challenges in APE, which basically can summarize from introduction)

\paragraph{The Need for a Comprehensive Framework.}
Despite these advances, current methods largely address specific aspects of prompt design (e.g., optimizing the task instruction or few-shot demonstrations~\cite{khattab2022demonstrate}) and
often remain disconnected from more complex, multi-node LLM architectures.
To our knowledge, there is currently no unified system that allows developers to build and optimize \emph{any} LLM application in a single environment.
\emph{LLMDiff}, integrated within the AdalFlow library, will be the first auto-grad system offering this level of flexibility---much like how PyTorch~\cite{paszke2019pytorch} and
TensorFlow~\cite{abadi2016tensorflow} can automatically differentiate any combination of basic neural networks (e.g., RNNs, CNNs, Transformers).
By unifying automatic differentiation, prompt optimization, and multi-node support under one coherent framework, LLMDiff provides a powerful new paradigm for large-scale LLM development.

